Quantum annular homology and bigger Burnside categories

As part of their construction of the Khovanov spectrum, Lawson, Lipshitz and Sarkar assigned to each cube in the Burnside category of finite sets and finite correspondences, a finite cellular spectrum. In this paper we extend this assignment to cubes in Burnside categories of infinite sets. This is later applied to the work of Akhmechet, Krushkal and Willis on the quantum annular Khovanov spectrum with an action of a finite cyclic group: we obtain a quantum annular Khovanov spectrum with an action of the infinite cyclic group.

==> aux/Bibliography.tex <==
%\addcontentsline{toc}{section}{References}
\begin{thebibliography}{20}

\bibitem{AKW21} R. Akhmechet, V. Krushkal and M. Willis (2021). Stable homotopy refinement of quantum annular homology, \textit{Compositio Math.} 157, 710–769

\bibitem{APS04} M. Asaeda, J. Przytycki and A. Sikora (2004). Categorification of the Kauffman bracket skein module of I-bundles over surfaces, \textit{Algebr. Geom. Topol.} 4, 1177-1210.

\bibitem{BPW19} A. Beliakova, K. Putyra, S. Wehrli (2019). Quantum Annular Link Homology via Trace Functor I, \textit{Invent. Math.} 215, 383-492

\bibitem{H02} A. Hatcher (2002). \textit{Algebraic topology}. Cambridge: Cambridge University Press.

\bibitem{HP89} J. Hoste and J. Przytycki (1989). An invariant of Dichromatic Links, \textit{Proceedings of the American Mathematical Society}, 105(4) 1003-1003.

\bibitem{K00} M. Khovanov (2000). A categorification of the Jones polynomial, \textit{Duke Math. J.} 101, no. 3, 359-426.

\bibitem{LLS17} Lawson, T., Lipshitz R. and Sarkar, S. (2021). The Cube and the Burnside Category. \textit{Categorification in geometry, topology, and physics}. 63-85, Contemp. Math., 684, Amer. Math. Soc., Providence, RI, 2017 

\bibitem{LLS19} Lawson, T., Lipshitz R. and Sarkar, S. (2019). Khovanov Homotopy Type, Burnside Category, and Products (2020). \textit{Geometry and Topology}, 24, 623-745.

\bibitem{LS14} R. Lipshitz and  S. Sarkar (2014). A Khovanov stable homotopy type. J. Amer. Math. Soc. \textbf{27}, 983-1042.

\bibitem{LSSpatial} Lipshitz R. and Sarkar, S. (2019). Spatial refinements and Khovanov homology. \textit{Proceedings of the ICM 2018}, 1153--1173.

\bibitem{ML71} Mac Lane, S. (1971). \textit{Categories for the working mathematician}. Springer-Verlag, New York. Graduate Texts in Mathematics, Vol. 5.

\bibitem{M71} T. Matumoto (1971). On {$G$}-{${\rm CW}$} complexes and a theorem of {J}. {H}. {C}. {W}hitehead, \textit{{J. Fac. Sci. Univ. Tokyo Sect. IA Math.}} 18, 363--374.

\bibitem{V02} O. Viro (2002). Remarks on definition of Khovanov homology.

\bibitem{V73} Vogt, R. M. (1973). Homotopy limits and colimits. \textit{Math. Z. 134}. 11-52

\bibitem{FTW73} Farrell, F. T. and Taylor, L. R. and Wagoner, J. B. (1973). The Whitehead theorem in the proper category. \text{Compositio Math. 27}. 1--23

\end{thebibliography}
